An Improved Local Search Algorithm for k-Median

We present a new local-search algorithm for the $k$-median clustering problem. We show that local optima for this algorithm give a $(2.836+\epsilon)$-approximation; our result improves upon the $(3+\epsilon)$-approximate local-search algorithm of Arya et al. [STOC 01]. Moreover, a computer-aided analysis of a natural extension suggests that this approach may lead to an improvement over the best-known approximation guarantee for the problem. The new ingredient in our algorithm is the use of a potential function based on both the closest and second-closest facilities to each client. Specifically, the potential is the sum over all clients, of the distance of the client to its closest facility, plus (a small constant times) the truncated distance to its second-closest facility. We move from one solution to another only if the latter can be obtained by swapping a constant number of facilities, and has a smaller potential than the former. This refined potential allows us to avoid the bad local optima given by Arya et al. for the local-search algorithm based only on the cost of the solution.

==> combine-AB.tex <==
\subsection{Far Case}

\subsubsection{Type \xA}
When $\rho \leq \nicefrac{2}{3}$, we have

\begin{align}
\Gsum{c} \leq {}& (1+\a\b)\, d^* - (1+\a\b)\, d_1\notag\\
 = {} & \hoono{1.6\, d^* - 1.6\, d_1}. \label{eqnapx:f11}
\end{align}

When $\nicefrac{2}{3} < \rho \leq \nicefrac{3}{4}$,  we have
\begin{align}
\Gsum{c} \leq {}& (\nicefrac{3}{4}(1+\a\b) + \nicefrac{1}{4}+\nicefrac{1}{4\rho} + \nicefrac{\b}{2})\, d^* - (1+\a\b +(\a\b-2\b-\nicefrac{1}{\rho})/4)\, d_1\notag\\
 ={} &(1 + \nicefrac{3\a\b}{4} +\nicefrac{\b}{2} + \nicefrac{1}{4\rho})\, d^* - (1+\nicefrac{5\a\b}{4} -\nicefrac{\b}{2} -\nicefrac{1}{4\rho})\, d_1\notag\\
 \leq {} & \hoono{1.925\, d^* - 1.275\, d_1}. \label{eqnapx:f12}
\end{align}

When $\rho > \nicefrac{3}{4}$,  we have
\begin{align}
\Gsum{c} \leq {}& (1+\nicefrac{3\a\b}{4} + \nicefrac{\b}{2} + \nicefrac{1}{4\rho} + (\nicefrac{3}{4}-\rho)(\b+\nicefrac{(1+\a\b)}{\rho}))\, d^*\notag\\
& - (1+\a\b + (\a\b-2\b-\nicefrac{1}{\rho})/4 +(\nicefrac{3}{4}-\rho)(\a\b-(1+\a\b)/\rho)\, d_1\notag\\
 \leq {} &(\nicefrac{5\b}{4}-\nicefrac{\a\b}{4}   + \nicefrac{1}{\rho} + \nicefrac{3\a\b}{4\rho} -\rho\b)\, d^* \notag\\
& - (2+3\a\b -\nicefrac{\b}{2} - \nicefrac{1}{\rho} - \nicefrac{3\a\b}{4\rho} - \rho\a\b)\, d_1\notag\\
\leq {} & \hoono{1.8833\, d^* - 1.316\, d_1}. \label{eqnapx:f13}
\end{align}


%\subsubsection{When $\eta_1 = else$, $\eta_2 = f_1$}

\subsubsection{Type \xB}

%\begin{mybox}
%\begin{align}
%\eta_1:\quad & ((1+\rho)(1+\a\b)+\b)\, d^* -((1-\rho)(1+\a\b)+\a\b)\, d_1\\
%\eta_2:\quad & (1+\a\b)\, d^* - (1+\a\b)\, d_1\notag\\
%T_1:\quad & (1+\rho + 2\b)\, d^* - (1+2\a\b -2\b - \rho )\, d_1\notag\\
%T_2:\quad & (1+\a\b)\, d^* - (1+\a\b)\, d_1
%\end{align}
%\end{mybox}


When $\rho \leq \nicefrac{2}{3}$,  we have

\begin{align}
\Gsum{c} \leq {}& (1+\rho + \nicefrac{3\b}{2} + \nicefrac{\a\b}{2} + \nicefrac{\rho\a\b}{2})\, d^* - (1+2\a\b-\rho -\b - \nicefrac{\rho\a\b}{2})\, d_1\notag\\
\leq {} &   \hoono{2.47\, d^* - 1.13\, d_1}. \label{eqnapx:f21}
\end{align}

When $\nicefrac{2}{3} < \rho \leq \nicefrac{3}{4}$,  we have
\begin{align}
\Gsum{c} \leq {}& (1+\nicefrac{3\rho}{4} + \nicefrac{3\a\b}{4} + \b +\nicefrac{\rho\a\b}{2})\, d^* - (1+\nicefrac{7\a\b}{4}-\nicefrac{\b}{2}-\nicefrac{3\rho}{4} -\nicefrac{\rho\a\b}{2})\, d_1\notag\\
\leq {} & \hoono{2.437\, d^* - 1.16\, d_1}. \label{eqnapx:f22}
\end{align}

When $\rho > \nicefrac{3}{4}$,  we have

Note the expected cost of  $\eta_2$-simple swap 
is less than the expected cost of $\eta_1$-simple swap
thus we can get the same bound leading to 
\begin{align}
\Gsum{c} \leq {}& (1+\nicefrac{3\a\b}{4} + \nicefrac{\b}{2} + \nicefrac{\rho}{4} + (\nicefrac{5}{4}-\rho)(\rho+\rho\a\b+\b))\, d^*\notag\\
& - (1+\a\b -\nicefrac{\rho}{4} +\nicefrac{\a\b}{4} -\nicefrac{\b}{2} +(\nicefrac{5}{4}-\rho)(-\rho-\rho\a\b+\a\b))\, d_1\notag\\
= {} & (1+\nicefrac{3\a\b}{4} + 1.75\b + 1.5\rho +\nicefrac{5\rho\a\b}{4}-\rho^2-\rho^2\a\b-\rho\b)\, d^*\notag\\
& - (1+2.25\a\b-1.5\rho+\nicefrac{\a\b}{4}-\nicefrac{\b}{2}-2.25\rho\a\b+\rho^2+\rho^2\a\b)\, d_1\notag\\
\leq {} & \hoono{2.4375\, d^* - d_1}. \label{eqnapx:f23}
\end{align}




\subsection{Close Case}

\subsubsection{Type \xA, when $\eta_1 = f_1$, $\eta_2 = else$.}

\textbf{When $f_1$ and $f_2$ belong to different trees}


When $\nicefrac{2}{3} < \rho \leq \nicefrac{3}{4}$, we have

\begin{align}
\Gsum{c} \leq {}& (1+\nicefrac{3\a\b}{4} + \nicefrac{\b}{2} + \nicefrac{5\b}{4\rho})\, d^* - (\nicefrac{5}{4} - \nicefrac{\b}{2} - \nicefrac{5\b}{4\rho})\, d_1 + (\nicefrac{1}{4}-\nicefrac{9\b}{4})\, d_2\notag\\
\leq {} & (1+\nicefrac{3\a\b}{4} + \nicefrac{\b}{2} + \nicefrac{5\b}{4\rho})\, d^* - (1 + 1.75\b - \nicefrac{5\b}{4\rho})\, d_1 \tag{$-d_2 \leq -d_1$}\\
\leq {} & \hoono{1.925\, d^* - 0.975\, d_1}. \label{eqnapx:c111}
\end{align}



When $\rho >\nicefrac{3}{4}$, we have

\begin{align}
\Gsum{c} \leq {}& (1+\nicefrac{\b}{\rho} + (\nicefrac{5}{4}-\rho)(\b+\a\b) + (\rho - \nicefrac{3}{4})(2\b+\nicefrac{\b}{\rho}) + \nicefrac{\a\b}{4} + \b/(4\rho))\, d^*\notag\\
& - (1-\nicefrac{\b}{\rho}+\rho -\b - \b\rho -\nicefrac{3}{4}+\nicefrac{3\b}{4}+\nicefrac{3\b}{4\rho} + \nicefrac{1}{4}-\nicefrac{\b}{2}-\nicefrac{\b}{4\rho} )\, d_1\notag\\
& + (-2.5\b +2\rho\b + \rho - 3\rho\b -\nicefrac{3}{4} +2.25\b-\nicefrac{\b}{4} +\nicefrac{1}{4}-\b)\, d_2\notag\\
= {}& (1+\nicefrac{3\b}{4}+\nicefrac{\b}{2\rho} + 1.5\a\b - \rho\a\b +\rho\b)\, d^* \notag\\
& - (0.5-\nicefrac{3\b}{4}-\nicefrac{\b}{2\rho}+\rho-\b\rho)\, d_1\notag\\
& - (0.5+1.5\b-\rho+\rho\b)\, d_2\notag\\
\leq {}& (1+\nicefrac{3\b}{4}+\nicefrac{\b}{2\rho} + 1.5\a\b - \rho\a\b +\rho\b)\, d^*\notag\\
& - (1+\nicefrac{3\b}{4}-\nicefrac{\b}{2\rho})\, d_1\tag{$-d_2 \leq -d_1$}\\
\leq {} & \hoono{1.884\, d^* - 1.02\, d_1}. \label{eqnapx:c112}
\end{align}


\textbf{When $f_1$ and $f_2$ belong to the same tree.}



When $\nicefrac{2}{3} < \rho \leq \nicefrac{3}{4}$, we have

\begin{align}
\Gsum{c} \leq {}& (\nicefrac{5}{4}+\nicefrac{3\a\b}{4} + \nicefrac{3\b}{4} + \nicefrac{\b}{2\rho} + \nicefrac{1}{4\rho})\, d^*\notag\\
& - (\nicefrac{5}{4} - \nicefrac{\b}{2\rho} - \nicefrac{3\b}{4} - \nicefrac{1}{4\rho})\, d_1
 - 1.75\b\, d_2\notag\\
\leq {} &  \hoono{2.375\, d^* - 0.925\, d_1}. \label{eqnapx:c121}
\end{align}



When $\rho >\nicefrac{3}{4}$, we have

\begin{align}
\Gsum{c}
\leq {} & (1+\nicefrac{\b}{2}+\nicefrac{\b}{2\rho}+(\nicefrac{5}{4}-\rho)(\a\b) + (\rho-\nicefrac{3}{4})(\b+\nicefrac{\b}{\rho})\notag\\
&  + \nicefrac{\a\b}{4} + \nicefrac{1}{4}+\nicefrac{\b}{4}+\nicefrac{1}{4\rho})\, d^*\notag\\
& - (1-\nicefrac{\b}{2\rho} + (\rho-\nicefrac{3}{4})(1-\b-\nicefrac{\b}{\rho}) + \nicefrac{1}{4}(1-3\b-\nicefrac{1}{\rho}))\, d_1\notag\\
& - (1.75\b - (\rho-\nicefrac{3}{4})(1-\b))\, d_2\notag\\
= {}& (\nicefrac{5}{4}+\b+\rho\b+1.5\a\b-\rho\a\b+\nicefrac{1}{4\rho}-\nicefrac{\b}{4\rho})\, d^*\notag\\
& - (0.5-\b+\nicefrac{\b}{4\rho}+\rho - \rho\b-\nicefrac{1}{4\rho})\, d_1\notag\\
& - (\b+\nicefrac{3}{4}-\rho+\rho\b)\, d_2\notag\\
\leq {} &  \hoono{2.317\, d^* - 0.98\, d_1}. \label{eqnapx:c122}
\end{align}


\subsubsection{Type \xB, When $\eta_1 = else$, $\eta_2 = f_1$}


\textbf{When $f_1$ and $f_2$ belong to different trees.}




When $\rho \leq \nicefrac{2}{3}$, we have

\begin{align}
\Gsum{c} \leq {}& (1+\b+2\rho\b)\, d^* - (2-1.5\b-2\rho\b)\, d_1 + (1-3.5\b)\, d_2\notag\\
\leq {} & (2-2.5\b-1.5\rho\b+\rho)\, d^* - (2-1.5\b+2\rho\b-\rho)\, d_1 \tag{$d_2\leq d^*+\rho(d^*+d_1)$}\\
\leq {} & \hoono{1.967\, d^* - 1.3\, d_1}. \label{eqnapx:c221}
\end{align}

When $\nicefrac{2}{3} < \rho \leq \nicefrac{3}{4}$,

\begin{align}
\Gsum{c} \leq {}& (1+\b + 1.75\rho\b+\nicefrac{\a\b}{4})\, d^* - (1.75-\b-1.75\rho\b)\, d_1 + (\nicefrac{3}{4}-2.75\b)\, d_2\notag\\
\leq {} & (1.75-1.75\b-\rho\b+\nicefrac{\a\b}{4}+\nicefrac{3\rho}{4})\, d^* - (1.75-\b+\rho\b-\nicefrac{3\rho}{4})\, d_1 \tag{$d_2\leq d^*+\rho(d^*+d_1)$}\\
\leq {} & \hoono{1.963\, d^* - 1.137\, d_1}. \label{eqnapx:c222}
\end{align}

When $\rho > \nicefrac{3}{4}$, we have

\begin{align}
\Gsum{c} \leq {}& (1+\nicefrac{\b}{2}+\rho\b + (\nicefrac{5}{4}-\rho)(\b+\rho\b) + (\rho-\nicefrac{3}{4})(\a\b) + \nicefrac{\a\b}{4} + \nicefrac{3\rho\b}{4})\, d^*\notag\\
& - (1-\nicefrac{\rho\b}{2} + (\nicefrac{5}{4}-\rho)(1-\b-\rho\b)+\nicefrac{1}{4}-\nicefrac{\b}{2}-\nicefrac{3\rho\b}{4})\, d_1\notag\\
& + (-1.5\b+ (\nicefrac{5}{4}-\rho)(1-\b) + \nicefrac{1}{4}-\nicefrac{3\b}{4})\, d_2\notag\\
= {} & (1+1.75\b+2\rho\b-\rho^2\b + \rho\a\b-0.5\a\b)\, d^* - (2.5-1.75\b-1.5\rho\b-\rho+\rho^2\b)\, d_1\notag\\
&  + (1.5-3.5\b-\rho+\rho\b)\, d_2\notag\\
\leq {} & (2.5-1.75\b -\nicefrac{5\rho\b}{4} +\nicefrac{\rho}{2} +\rho\a\b-0.5\a\b-\rho^2+\rho^2\b)\, d^*\notag\\
&  - (2.5-1.75\b+2\rho\b-2.5\rho+\rho^2)\, d_1\tag{$d_2\leq d^*+\rho(d^*+d_1)$}\notag\\
\leq {} & \hoono{2.0375\, d^* -1.05\, d_1}. \label{eqnapx:c223}
\end{align}



\textbf{
When $f_1$ and $f_2$ belong to the same tree.}


When $\rho \leq \nicefrac{2}{3}$, we have

\begin{align}
\Gsum{c} \leq {}& (1.5+1.5\b+\rho\b + \nicefrac{\rho}{2})\, d^* - (2-2\b-\rho\b-\nicefrac{\rho}{2})\, d_1 + (0.5-2.5\b)\, d_2\notag\\
\leq {} & \hoono{2.27\, d^* - 1.13\, d_1}. \label{eqnapx:c211}
\end{align}

When $\nicefrac{2}{3} < \rho \leq \nicefrac{3}{4}$, we have

\begin{align}
\Gsum{c} \leq {}& (\nicefrac{5}{4} + \nicefrac{5\b}{4} + \rho\b + \nicefrac{\rho}{4} + \nicefrac{\a\b}{4})\, d^*\notag\\
& - (1.75 - \nicefrac{5\b}{4} - \rho\b - \nicefrac{\rho}{4})\, d_1 + (0.5-2.25\b)\, d_2\notag\\
\leq {} & (1.75-\b -\nicefrac{5\rho\b}{4} + \nicefrac{3\rho}{4} + \nicefrac{\a\b}{4})\, d^*\notag\\
& - (1.75-\nicefrac{5\b}{4} +\nicefrac{5\rho\b}{4} -\nicefrac{3\rho}{4})\, d_1\notag\\
\leq {} & \hoono{2.075\, d^*-1.125\, d_1}. \label{eqnapx:c212}
\end{align}


When $\rho> \nicefrac{3}{4}$, we have
\begin{align}
\Gsum{c} \leq {}& (\nicefrac{5}{4}+\nicefrac{3\b}{4} + \nicefrac{\rho\b}{2} + (\nicefrac{5}{4}-\rho)(\b+\rho\b) + \rho\a\b + \nicefrac{\rho}{4}-0.5\a\b)\, d^*\notag\\
& - (1-\nicefrac{\rho\b}{2} + (\nicefrac{5}{4}-\rho)(1-\b-\rho\b) + \nicefrac{1}{4}-\nicefrac{3\b}{4}-\nicefrac{\rho}{4})\, d_1\notag\\
& - (\b + (\nicefrac{5}{4}-\rho)(\b-1) + \nicefrac{3\b}{4})\, d_2\notag\\
={}  & (\nicefrac{5}{4}+2\b+\nicefrac{3\rho\b}{4} - \rho^2\b +\rho\a\b - 0.5\a\b +\nicefrac{\rho}{4})\, d^*\notag\\
& - (2.5-\nicefrac{3\rho\b}{4}-2\b-\nicefrac{5\rho}{4}+\rho^2\b )\, d_1 - (3\b-\nicefrac{5}{4}-\rho\b+\rho)\, d_2\notag\\
\leq {} & (1.345 + \rho - 0.2\rho^2)\, d^* - (2.1-1.4\rho+0.2\rho^2)\, d_1 + (0.65 - 0.8\rho)\, d_2\notag
\end{align}

If $\rho \leq 0.8125$, then $d_2 \geq 0$. Thus we get 
\begin{align}
\Gsum{c} \leq \hoono{2.07\, d^* - 1.09\, d_1}. \label{eqnapx:c2131}
\end{align}

If $\rho > 0.8125$, then $d_2 < 0$. Thus we get 
\begin{align}
\Gsum{c} \leq \hoono{2.15\, d^* - 1.05\, d_1}\label{eqnapx:c2132}
\end{align}


%\iffalse
%
%
%\david{I think the threshold is $\rho \leq 0.86875$ instead of $0.8125$}
%For $\rho \leq 0.86875$, the coefficient of $d_2$ is nonnegative when multiplied with corresponding probability matrix, so we replace $d_2$ with $d^* + \rho(d^*+d_1)$.
%$C = 
%\begin{bmatrix} 1.8+0.8\rho& 1.4-0.2\rho & 1.8+0.6\rho & 1.4-0.2\rho \notag\\
% 1.8-0.8\rho & 1 + 0.2\rho & 1.4-0.6\rho & 1+0.2\rho\end{bmatrix} $
% % \begin{bmatrix} 2+\rho& 1.4-0.2\rho \notag\\ 1.8+0.6\rho & 1.4-0.2\rho \end{bmatrix} ,
% % \begin{bmatrix} 1.8-\rho & 1 + 0.2\rho \notag\\ 1.4-0.6\rho & 1+0.2\rho\end{bmatrix} $
%
%Otherwise we replace $d_2$ with $d_1$ to get 
%$C' =
%\begin{bmatrix} 1.4+0.4\rho& 1.8+0.2\rho & 2.2+\rho & 1.6\notag\\
%  1.4+0.4\rho & 1.4-0.2\rho & 1.8-\rho & 1+0.2\rho\end{bmatrix} $
% % \begin{bmatrix} 1.4+0.4\rho& 1.8+0.2\rho \notag\\ 2.2+\rho & 1.6\end{bmatrix} ,
% % \begin{bmatrix} 1.4+0.4\rho & 1.4-0.2\rho \notag\\ 1.8-\rho & 1+0.2\rho\end{bmatrix} $
%
%
%\david{case $\nicefrac{2}{3}$ useless, by assumption of lemma}
%\begin{itemize}
%%\item Case $\rho \leq \nicefrac{2}{3}:$ We get $C\cdot P_{\nicefrac{2}{3}} \leq $
%%% we can combine the $\eta_1$ simple swap and the $\eta_1$-tree swap, then the coefficient of $d_2$ is 0.
%%$
%%\begin{bmatrix} 2.333 & \cdot & 2.2 & \cdot \notag\\
%%   1.2666 & \cdot & 1& \cdot \end{bmatrix} \cdot P_{\nicefrac{2}{3}}
%% % \begin{bmatrix} 2.2667 & \cdot \notag\\ 2.2 & \cdot \end{bmatrix} ,
%% % \begin{bmatrix}  1.133 & \cdot \notag\\ 1& \cdot \end{bmatrix} 
%% \leq \begin{bmatrix} 2.2665\notag\\ 1.1333\end{bmatrix} $
%
%\item Case $\nicefrac{2}{3}<\rho \leq \nicefrac{3}{4}:$ We get $C\cdot P_{\nicefrac{3}{4}}\leq $
%$\begin{bmatrix} 2.4 & \cdot & 2.25 & 1.27 \notag\\
%   1.2 & \cdot & 0.95 & 1.13\end{bmatrix}  \cdot P_{\nicefrac{3}{4}}
% % \begin{bmatrix} 2.75 & \cdot \notag\\ 2.25 & 1.27 \end{bmatrix} 
% % \begin{bmatrix}  1.05 & \cdot \notag\\ 0.95 & 1.13\end{bmatrix} 
% \leq \begin{bmatrix} 2.08\notag\\ 1.12\end{bmatrix} $.
%
%%$d_2$ becomes negative when $(2.5-2\rho)(1-2\b)+(2\rho-1.5)(-2\b)-1.5\b \leq 0 \Rightarrow \rho \geq 0.8125$
%\item Case $\nicefrac{3}{4}<\rho \leq 0.86875:$ We get $C\cdot P_{1} \leq
%\begin{bmatrix} 2.5 & \nicefrac{5}{4} & 2.322 & \nicefrac{5}{4} \notag\\
%  1.105 & 1.15 & 0.87875& 1.15\end{bmatrix} \cdot P_{1}
% % \begin{bmatrix} 2.8125 & \nicefrac{5}{4} \notag\\ 2.2875 & \nicefrac{5}{4} \end{bmatrix} 
% % \begin{bmatrix} 0.9875 & 1.15 \notag\\ 0.9125& 1.15\end{bmatrix} 
% \leq\begin{bmatrix} 2.14\notag\\ 1.05\end{bmatrix} $ (opt is maximized when $\rho = \nicefrac{3}{4}$, alg minimized when $\rho = \nicefrac{3}{4}$
%\item $\rho > 0.86875: \quad C' \cdot P_1 \leq
%\begin{bmatrix} 1.8 & 2 & 3.2 & 1.6 \notag\\
%  1.4 & 1.2 & 0.8 & 1 \end{bmatrix} \cdot P_1
% \leq \begin{bmatrix} 2.15\notag\\  1\end{bmatrix} $
% % \begin{bmatrix} 1.8 & 2 \notag\\ 3.2 & 1.6 \end{bmatrix} 
% % \begin{bmatrix} 1.4 & 1.2 \notag\\ 0.8 & 1 \end{bmatrix} 
% % \leq (2.15, 1)$
%
%\end{itemize}
%
%\fi



